Distributed Quantum Learning with co-Management in a Multi-tenant Quantum System

The rapid advancement of quantum computing has pushed classical designs into the quantum domain, breaking physical boundaries for computing-intensive and data-hungry applications. Given its immense potential, quantum-based computing systems have attracted increasing attention with the hope that some systems may provide a quantum speedup. For example, variational quantum algorithms have been proposed for quantum neural networks to train deep learning models on qubits, achieving promising results. Existing quantum learning architectures and systems rely on single, monolithic quantum machines with abundant and stable resources, such as qubits. However, fabricating a large, monolithic quantum device is considerably more challenging than producing an array of smaller devices. In this paper, we investigate a distributed quantum system that combines multiple quantum machines into a unified system. We propose DQuLearn, which divides a quantum learning task into multiple subtasks. Each subtask can be executed distributively on individual quantum machines, with the results looping back to classical machines for subsequent training iterations. Additionally, our system supports multiple concurrent clients and dynamically manages their circuits according to the runtime status of quantum workers. Through extensive experiments, we demonstrate that DQuLearn achieves similar accuracies with significant runtime reduction, by up to 68.7% and an increase per-second circuit processing speed, by up to 3.99 times, in a 4-worker multi-tenant setting.

==> background.tex <==
\section{Background}
A Generative Adversarial Network (GAN) broadly refers to an architecture comprised of two models which compete against one and other, playing an adversarial game. Each model is tasked with attempting to fool the other in a game of cat and mouse \cite{goodfellow2014generative}. The common example of the generator being a fraudster producing fake money (generator), wanting to fool a detective (discriminator) who is trained in discerning between fake and real money. The GAN architecture typically consists of a real data set $(x)$, a Discriminator (D) and a Generator (G). The discriminator's objective is to be able to correctly classify between real and fake data synthesized by G. The generator's objective is to synthesize samples that the discriminator will classify as real. 
%This generic architecture is visualized in Figure \ref{fig:highlevelgan}.


%\begin{figure}[!htb]
%\centering
%         \includegraphics[width=0.7\linewidth]{figs/BasicGANArch.jpg}
      %\vspace{-0.35in}
%\caption{High Level GAN Architecture}
%      \label{fig:highlevelgan}
%      \vspace{-0.3cm}
%\end{figure}

With this architecture being rather generic, GANs are agnostic of the type of data they are fed and have applications in an extensive set of domains. However, the performance within each respective application is strongly dictated by the network architecture \cite{wang2019generative}. GANs have shown exceptional results in, but not limited to, computer vision \cite{wang2019generative} and time-based domains such as music composition \cite{dong2018musegan}. In traditional generative networks, G samples from a specific distribution $p_z$ to synthesize a fake sample which is to be fed to D. D is fed with both real data $x$ and data synthesized by G. The discriminator's output is a perception on the data that is fed, and its goal is to maximize $D(x)$  and to minimize $D(G(p_z))$. While the generator's goal is to maximize $D(G(p_z)$. Where probabilistic models aim to label real data as 1 and fake data as 0, the primal min-max optimization formulation is described in Equation \ref{eqn:lossfunc}.

\begin{equation}
\begin{split}
    min_G max_D V(D,G) = \mathbf{E}_{x\text{~}{p}_{data(x)} }[log(D(x)] + \\ \mathbf{E}_{z\text{~}{p}_z(z)}[log(1-D(G(z))]
\end{split}
\label{eqn:lossfunc}
\end{equation}

The one direction in relation to the GAN-related research is to explore the potential of quantum GANs \cite{huang2020experimental,hu2019quantum,lloyd2018quantum}. The conceptual translation between a classical GAN and a quantum GAN is relatively intuitive, as the generator network's task is to learn the underlying probability distribution of a real data set and quantum computers produce probability distributions instead of discrete values. Prior studies propose the use of quantum GANs ranging from for attempting to attain a quantum speed up, or for data loading onto quantum computers %\cite{lloyd2018quantum,hu2019quantum,zoufal2019quantum,verdon2019learning,beer2020training,chen2019variational}
\cite{zoufal2019quantum,beer2020training,chen2019variational,verdon2019learning}. For example, Zoufal et al.~\cite{zoufal2019quantum} present Qi-GAN to learn random distributions for financial applications. Their work, however, is only extended to one dimensional data learning, and displays significant instability within their models evaluation. Furthermore, they make use of a classical discriminator, and hence making their Qi-GAN only a partial quantum GAN that might not be fully accelerated by quantum systems. Another example of a Quantum GAN~\cite{dallaire2018quantum} makes the use of variational circuits. The authors present a Quantum GAN architecture. However, their learning is rather sporadic and inconsistent, with a non-convergent and  unclear trend. 

Based on the quantum state fidelity based loss functions for Generator and Discriminator,  we propose QuGAN that  provides a more stable and scalable architecture of quantum GANs. 

\subsection{Quantum Fidelity Measurement}

One crucial component regarding the proposed Quantum GAN (QuGAN) architecture is the SWAP test, a quantum state fidelity algorithm. Two states, $|\phi\rangle$ and $|\psi\rangle$, are passed to a system where the measured output is their fidelity. One anicilla qubit in state $\frac{1}{\sqrt{2}}|0\rangle + \frac{1}{\sqrt{2}}|1\rangle$ is passed to the system along side the aforementioned states. The quantum state is described in Equation~\ref{eqn:initial_swap_test_state}.

\begin{equation}
    State = \frac{1}{\sqrt{2}}|0,\phi,\psi\rangle + \frac{1}{\sqrt{2}}|1,\phi,\psi\rangle
    \label{eqn:initial_swap_test_state}
\end{equation}

Following this, the algorithm makes use of a control swap gate, where if the control qubit measures 1 the states are swapped, otherwise nothing happens. The state of $|\psi\rangle$ and $|\phi\rangle$ are control swapped with the anicilla qubit as the control qubit, resulting in the state described in Equation~\ref{eqn:mid_swap_test_state}.

\begin{equation}
\begin{split}
        State = \frac{1}{\sqrt{2}}|0,\phi,\psi\rangle + 
        \frac{1}{\sqrt{2}}|1,\psi,\phi\rangle
    \label{eqn:mid_swap_test_state}
    \end{split}
\end{equation}

The anicilla qubit is passed through a Hadamard gate referenced in Equation \ref{eq:had}, placing the system in the state described in Equation \ref{eqn:post_hadamard}.

\begin{equation} 
H=\left[\begin{array}{cc}
\frac{1}{\sqrt{2}} & \frac{1}{\sqrt{2}} \\
\frac{1}{\sqrt{2}} & -\frac{1}{\sqrt{2}} 
\end{array}\right]
\label{eq:had}
\end{equation}


\begin{equation}
\begin{split}
        State = \frac{1}{2}(|0,\phi,\psi\rangle + |1,\phi,\psi\rangle +
        |0,\psi,\phi\rangle - |1,\psi,\phi\rangle 
 \end{split}
\label{eqn:post_hadamard}
\end{equation}

To attain the probability of measuring the anicilla qubit as 0, we square sum the states where $|0\rangle$ is measured.

\begin{equation}
\begin{split}
    State = \frac{1}{2}|0\rangle(|\phi\rangle|\psi\rangle + |\psi\rangle|\phi\rangle) +  \frac{1}{2}(|\phi\rangle|\psi\rangle - |\psi\rangle|\phi\rangle)
 \end{split}
    \label{eqn:state_based}
\end{equation}

To attain Equation~\ref{eqn:final_probability_swap}, we isolate the coefficients to the $|0\rangle$ state and square them to attain a P(Measurement=0), as seen in Equation \ref{eqn:state_based}. As described in Equation \ref{eqn:final_probability_swap},  the fidelity of states $|\phi\rangle$ and $|\psi\rangle$ is bound to [0.5,1], and measures the fidelity of two states. In the case of the states being orthogonal, the dot product between the matrices will equal 0 and the fidelity measures 0.5, and if the matrices are identical the dot product measures 1 and the fidelity measures 1.

\begin{equation}
    P(Measurement=0) = \frac{1}{2} + \frac{1}{2}|\langle\psi,\phi\rangle|^2
    \label{eqn:final_probability_swap}
\end{equation}
